A Benchmarking Study to Evaluate Apache Spark on Large-Scale Supercomputers

As dataset sizes increase, data analysis tasks in high performance computing (HPC) are increasingly dependent on sophisticated dataflows and out-of-core methods for efficient system utilization. In addition, as HPC systems grow, memory access and data sharing are becoming performance bottlenecks. Cloud computing employs a data processing paradigm typically built on a loosely connected group of low-cost computing nodes without relying upon shared storage and/or memory. Apache Spark is a popular engine for large-scale data analysis in the cloud, which we have successfully deployed via job submission scripts on production clusters. In this paper, we describe common parallel analysis dataflows for both Message Passing Interface (MPI) and cloud based applications. We developed an effective benchmark to measure the performance characteristics of these tasks using both types of systems, specifically comparing MPI/C-based analyses with Spark. The benchmark is a data processing pipeline representative of a typical analytics framework implemented using map-reduce. In the case of Spark, we also consider whether language plays a role by writing tests using both Python and Scala, a language built on the Java Virtual Machine (JVM). We include performance results from two large systems at Argonne National Laboratory including Theta, a Cray XC40 supercomputer on which our experiments run with 65,536 cores (1024 nodes with 64 cores each). The results of our experiments are discussed in the context of their applicability to future HPC architectures. Beyond understanding performance, our work demonstrates that technologies such as Spark, while typically aimed at multi-tenant cloud-based environments, show promise for data analysis needs in a traditional clustering/supercomputing environment.

==> additions.tex <==
\section{Abstract}\label{abstract}

In the spirit of software engineering, I have applied the separation of
concerns principle by creating a separate document for the abstract,
\href{http://drive.google.com/open?id=1lTxG_WOtMI6IbK3NU-cFe6LAKrQKN53Jn0MwpE7m3Xg}{\emph{Big
Data Processing in Apache Spark (Abstract)}}, since we have to submit it
separately. I'm going to work on actual paper organization and content
before Thursday.

\section{Overview}\label{overview}

Our goal is to understand and articulate the characteristics of
cloud-based dataflow processing in the context of HPC analysis tasks,
implement sample apps using spark, pegasus, and mpi and evaluate their
performance on both a supercomputing cluster and a cloud.

We will compare XYZ written in Apache Spark vs. MPI (a traditionally
used messaging middleware)

The benchmarks are chosen based on typical
computation/communication patterns found in HPC.

We're also looking at Python vs. Scala and whether there are any
performance differences.

Some words about tuning garbage collection. These folks seem to have
done some good legwork on same\footnote{https://databricks.com/blog/2015/05/28/tuning-java-garbage-collection-for-spark-applications.html}.

Also simply describe differences between implementation (e.g. lines of
code).

Out of core: Implicit in Spark

NOTE: we need to clarify what we mean by \emph{dataflow.}

\begin{itemize}
\item
  \begin{quote}
  Use in compilers:
  \href{https://en.wikipedia.org/wiki/Data-flow_analysis}{\emph{https://en.wikipedia.org/wiki/Data-flow\_analysis}}
  \end{quote}
\item
  \begin{quote}
  Dataflow architecture,
  https://en.wikipedia.org/wiki/Dataflow\_architecture
  \end{quote}
\end{itemize}

\section{Project Resources}\label{project-resources}

\textbf{Github:}
\href{http://github.com/cchriste/dataflow}{\emph{http://github.com/cchriste/dataflow}}

\textbf{Slack:}
\href{https://dataflowanalysis.slack.com}{\emph{https://dataflowanalysis.slack.com}}

\textbf{Google Docs:}
\href{https://drive.google.com/folderview?id=0BxLkEMNd9q6FfmpRaFZXSGlPc0JsSDdVdndCUm83SzN6UnlLVEk5T3ZsZmJ0VEVGREtNTkE\&usp=sharing}{\emph{dataflow\_analysis}}

\textbf{Dropbox:}
\href{https://www.dropbox.com/sh/odsd9uxe1elbhbf/AAD8J1TGuFY1VHJl2oPdm5E0a?dl=0}{\emph{spark\_hpc}}

My dropbox id is gkt@cs.luc.edu

\section{Dataflows}\label{dataflows}

\subsection{Components/Pipeline Stages}\label{componentspipeline-stages}

\begin{itemize}
\item
  \begin{quote}
  map
  \end{quote}
\item
  \begin{quote}
  flatmap
  \end{quote}
\item
  \begin{quote}
  reduce
  \end{quote}
\item
  \begin{quote}
  reducemap (ex: aggregation for file i/o)
  \end{quote}
\item
  \begin{quote}
  other?
  \end{quote}
\end{itemize}

\subsection{Multistage}\label{multistage}

Result of one computation feeds into the next, for example a \emph{map}
to another \emph{map}.

\subsection{Streaming}\label{streaming}

Computation performed over moving window.

\subsection{Evaluating Performance}\label{evaluating-performance}

Assessing the various components based on their rates of production and
consumption.

\subsection{To DAG or not to DAG}\label{to-dag-or-not-to-dag}

Some dataflows can have feedback..

\section{Dataflow Processing
Frameworks}\label{dataflow-processing-frameworks}

\subsection{Spark}\label{spark}

Spark is a general purpose cluster computing system similar to Hadoop.
It provides a new data abstraction that facilitates fast sharing and
history-based resilience, as well as an expanded set of data
transformation and actions, in addition to traditional map-reduce. In
addition, Spark provides a streaming processing abstraction as well as
bindings to common processing languages such as GraphX, R, and MLlib.

Spark is \emph{lazy,} and this philosophy underlies much of its design.
Computations will not be performed until their result is requested and
data will not be consolidated or repartitioned unless explicitly
requested.

\subsubsection{Running}\label{running}

Basics of job submission and execution.

\href{https://docs.google.com/document/d/1fq3z1-oEcCBhjKA__vl8LsVm3-uArJik7YFLYvYoN1Y/edit?usp=sharing}{\emph{running
spark on cooley}}

\href{https://docs.google.com/document/d/1lyzEHap1EznES0DKiMa3fsalepqPD6vnbZqSEMjCVPQ/edit?usp=sharing}{\emph{running
spark on magellan}}

\subsubsection{Resilient Distributed
Data}\label{resilient-distributed-data}

When a dataset is loaded by Spark, it becomes an immutable RDD. This
abstraction allows the data to be treated as a whole when in fact it may
be partitioned across many nodes of a distributed system. Each partition
also contains the history of transformations with which it was created,
called a \emph{lineage}, with which the partition can be recomputed if
necessary, such as in the case of a node failure. This lineage is a more
compact form of resiliency compared to data duplication as utilized by
Hadoop.

An RDD is split into \emph{partitions} whose size is at minimum the size
of a block on whatever storage device is being utilized (e.g. 32MB).
Each partition is further divided into \emph{records}, typically a
single line for text processing, or an entire binary file for binary
data. Binary data records can be explicitly specified. Large binary
files will be broken down into multiple partitions only if these
partitions can themselves be divided into records.

Spark distributes the blocks/data among the workers, if it does at all.

o is RDD different than Tachyon or do RDD blocks get written using
Tachyon (or HDFS, etc)?

o what data models does it support?

o how does it handle fault tolerance?

o what about transformation/views? (rows vs columns, more generally
chunks/blocks)

o when/how is the data replicated?

\subsubsection{}\label{section}

\paragraph{Storage Levels}\label{storage-levels}

RDDs can be stored in memory, on disk, a combination of the two, or off
heap (using Tachyon). MEMORY\_ONLY

Partitions that do not fit in memory will be recomputed from their
history when they are needed.

\subparagraph{DISK\_ONLY}\label{diskux5fonly}

All partitions are stored on disk, just like Hadoop.

RDD partitions can be optionally replicated across up to two nodes. An
RDD partition must be small enough to fit

\paragraph{Persistence}\label{persistence}

RDDs can be persisted in memory for fast access between successive
operations. This is particularly important for iterative algorithms that
reuse some intermediate result. An RDD will be persisted according to
its specified storage level. Caches are cleared according to a least
recently used policy, or manually using RDD.unpersist()

\paragraph{Input}\label{input}

In order to get binary data into spark, we use the binaryFiles or
binaryRecords SparkContext functions. Both will read a directory filled
with binary files. The first will create one record per file, while the
second will partition files into records of an explicitly stated number
of bytes. For example, the following line will create an RDD with
partitions containing records of size float{[}3{]}:

vecs = sc.binaryRecords(sys.argv{[}1{]}, 12)

The binary data is read into a string. If you want to use the data as a
numpy array, the numpy.fromstring function can be used:

arr= np.fromstring(vec, dtype=np.float32)

This function can be used by RDD.map in order to convert the string
records into numpy records:

data = vecs.map(parseVector)

\subsubsection{Streaming}\label{streaming-1}

How to run spark in streaming mode.

\subsubsection{Spark and Tachyon}\label{spark-and-tachyon}

How do they work together? Are the performance characteristics
different?

Is it the same as ceph on Magellan? (ask Dan Olsen about ceph)

\subsection{Pegasus}\label{pegasus}

todo

\subsection{MPI}\label{mpi}

todo: reference implementation

\section{System Architectures}\label{system-architectures}

\subsection{Cooley}\label{cooley}

225Tflop cluster with 40Tb memory, shared disk + 355Tb local disk per
node, ...

\subsection{Magellan}\label{magellan}

7000 node cloud, no shared disk, per-node provisioning flexibility,
\ldots{}

\section{Sample Applications}\label{sample-applications}

\subsection{APS}\label{aps}

\begin{enumerate}
\def\labelenumi{\arabic{enumi}.}
\item
  \begin{quote}
  analyze image stacks from advanced photon source
  \end{quote}
\item
  \begin{quote}
  save results as IDX
  \end{quote}
\end{enumerate}

Our first sample application comes from a materials scientist who
utilizes the Advanced Photon Source (APS) to scan the construction of a
polymer material that could be used for nanoscale circuit printing. We
received an image stack from the APS as well as a sample Matlab script
and reproduced the results using the Spark framework.

Details can be found here.

\subsection{Bioinformatics}\label{bioinformatics}

\begin{enumerate}
\def\labelenumi{\arabic{enumi}.}
\item
  \begin{quote}
  look for patterns in genome streams
  \end{quote}
\item
  \begin{quote}
  and stuff
  \end{quote}
\end{enumerate}

\subsection{EVS}\label{evs}

\begin{enumerate}
\def\labelenumi{\arabic{enumi}.}
\item
  \begin{quote}
  look for patterns in genome streams
  \end{quote}
\item
  \begin{quote}
  and stuff
  \end{quote}
\end{enumerate}

\section{Evaluation}\label{evaluation}

\subsection{Pipeline Benchmarks}\label{pipeline-benchmarks}

\begin{itemize}
\item
  \begin{quote}
  map
  \end{quote}
\item
  \begin{quote}
  flatmap
  \end{quote}
\item
  \begin{quote}
  reduce
  \end{quote}
\item
  \begin{quote}
  reducemap (ex: aggregation for file i/o)
  \end{quote}
\item
  \begin{quote}
  other?
  \end{quote}
\end{itemize}

\subsection{Application Benchmarks}\label{application-benchmarks}

- data sizes

- data rates

- \# of stages

- system scale

- M:N coupling (in flatmaps/reducemaps, fan-in/fan-out degress)

- hw

- spilling?

- magellan vs cooley (shared storage vs node-level storage)

\section{Meeting Notes}\label{meeting-notes}

\emph{17Jun}

1.
\href{https://docs.google.com/document/d/1fq3z1-oEcCBhjKA__vl8LsVm3-uArJik7YFLYvYoN1Y/edit?usp=sharing}{\emph{spark
on cooley}}

- verify number of threads is actually correct, that we can
control/monitor threading

o identify multiple threads/worker

- try to load binary data (aps data or bio data)

o partition a huge binary file

o load a directory of smaller binary files

- use /projects/SDAV/cam directory, which is persistent

note: file(s) must be accessible to all workers, either through shared
path or hdfs/tachyon/etc

- when multiple files are read (or one big file is split) where does the
data go?

- dissect RDD (esp in context of binary blob):

o is RDD different than Tachyon or do RDD blocks get written using
Tachyon (or HDFS, etc)?

o what data models does it support?

o how does it handle fault tolerance?

o what about transformation/views? (rows vs columns, more generally
chunks/blocks)

o when/how is the data replicated?

- explore pipelines

1b.
\href{https://docs.google.com/document/d/1lyzEHap1EznES0DKiMa3fsalepqPD6vnbZqSEMjCVPQ/edit?usp=sharing}{\emph{spark
on magellan}}

- ceph (distributed file system looking thing, ask Dan Olsen about it)

- ...

2. spark streaming, pipelines

articulate pipeline stages (benchmarks):

- map

- flatmap

- reduce

- reducemap (e.g. aggregation for file i/o)

- ?

once we introduce, it makes sense to talk about rates of production and
consumption for each pipeline component, and how we can make them work
together sanely ("frame dropping", etc)

- add another stage, now rates of production/consumption matter

evaluate (application benchmarks):

- data sizes

- data rates

- \# of stages

- system scale

- M:N coupling (in flatmaps/reducemaps, fan-in/fan-out degress)

- hw

- spilling?

- magellan vs cooley (shared storage vs node-level storage)

3. plan for summer

- Try a real problem on both cooley and magellan, compare pros and cons.

- ideas: aps data analysis, biology data, and even convert it to idx at
the end and attach a visus viewer.

- could use an existing spark analysis (such as their machine learning
module), or create our own

Understanding the overall system and tradeoffs and how cloud-iness can
help hpc will be a good contribution.

- could also have an mpi app that does the same thing to compare
performance

week 3-7 - explore and code

week 8-9 - benchmarking (aps, bioinformatics, or both)

week 10 - write report/paper

w3:

- google doc

- pipelines/streaming investigation

- spark running on Magellan

- binary data importing and RDD dissection

w4:

- start APS/BIO

- pipelining/streaming benchmark

- explore pegasus a little. We know the project lead (Eva Delman) so we
can ask questions. This is mainly to have a notion of related work.

- rdd vs tachyon?

w5:

- refine aps/bio app

- identify analyses

w6:

- 2nd app (either the aps or the bio)

- (spillover from prev weeks)

w7:

- finish and have working apps

\emph{15Jun}

Pegasus mpi*, Legion, Uintah task graph,

Create a simulator using mpi/spark, try different dataflows

Different "feeds" produce at different rates,

Have different "coupling" characteristics (\#consumers vs producers)

Different primitives (join, scatter, etc)

Streaming (small chunks), dataflow (overall processing task)

Can we create a benchmark to characterize these types of *in-memory*
pipelines using these building blocks with their given characteristics?

Including not only dag but also feedback loops.

Challenge is to separate performance from effectiveness of pipeline.

We can try this using both spark and Pegasus using Cooley and Magellan.

Magellan has a lot of flexibility in configuration, so we could even
using it to test heterogeneous frameworks.

We're going to let some task graph scheduler decide how to schedule the
Dataflow (default spark and Pegasus ways).

We want to explore dynamic modification of pipelines (eg add a new
processing node) and speculate as to what Api would be required to
facilitate this (ex: pause upstream then insert node then resume).

We'll generate examples from meta genomics for which we have in house
operations, we could also try climate.

First we'll try sample data to debug: gen a big 1d array, compute sum of
each successive pair, etc

Google doc to track thoughts


==> delete/discussion.tex <==



==> delete/introduction.tex <==
\section{Introduction}

In this early experience paper, our ultimate goal is to understand and articulate the characteristics of cloud-based dataflow processing in the context of HPC analysis tasks, implement sample apps using Spark and MPI and evaluate their performance on both a supercomputing cluster and in a high-performance cloud. Here we focus our efforts on a micro-benchmark that can be used to understand strong and weak scaling using two of the preferred development languages for Spark: Python and Scala.

In our experience, many data-intensive MPI programs follow a typical pattern: data loading/generation phase, perform a one or more computations on the data (possibly transforming it in the process) and performing a global operation in each step to get a final result. 

The workflow described above is found in many applications, including image processing. Consider for example a set of images to be analyzed (over time). An application would load the image data. The image data could be transformed (for example, color space transformation for feature extraction). An operation would be performed in place on the pixels to identify one or more features. Finally, information about the presence/absence of a feature across all images would be reported.

Thus we chose to create a micro-benchmark based on abstracting away details of this while ensuring that the actual workload would be realistic and reproducible in real world situations.

In addition, we wanted to understand whether the languages supported by Apache Spark play a role. The two main choices likely to be of interest to traditional HPC developers are Python and Scala (a promising JVM-based language with characteristics similar to Python but with ahead-of-time compilation as found in Java, C, and C++). We'll speak more to the affordances and constraints of these two choices in general, especially when it comes to use in Apache Spark, but we are encouraged by the results we are seeing in both of these approaches.

%\todo{Will probably defer the discussion of GC to a future paper. I don't think it is playing a role, because Apache Spark is providing a layer of abstract above GC to evict RDDs when needed to free up memory.}
%Some words about tuning garbage collection. These folks seem to have done some good legwork on same\footnote{https://databricks.com/blog/2015/05/28/tuning-java-garbage-collection-for-spark-applications.html}.

We're also intrigued by Apache Spark for software engineering reasons, namely the potential for developers to be productive without making a significant compromise to performance. While the story of Java and HPC is a long--and somewhat troubled--one, dating back to the Java Grande Forum effort and one of the author's previous efforts, the recent work on OpenJDK and Oracle's Java implementation have been progressively improving in performance. Notably, JVM startup time (which often leads to exaggerated impressions of bad performmance) has improved noticeably in recent iterations and is expected to continue improving with more regular updates to the Java Platform.

Another affordance of Apache Spark is its innate support for of out-of-core execution \emph{implicitly} and \emph{by default}. With its support for various strategies to cache to RAM, to disk, and even com
binations of the two, this is something that is simply not possible in traditional ahead-of-time (C) compiled environments without essentially reproducing many of the ideas of the Java Virtual Machine or building a memory-management framework (or by using memory caching services, e.g. memcached). Our benchmark has been designed to allow for \emph{data spilling} by adjusting any of the benchmark parameters (blocks, block size, or the partition multiplier). We'll speak to these issues in the detailed technical discussion.

Lastly, we wish to clarify what is meant when we use the term \emph{data flows}. A data flow in Apache Spark is where a data set is used to create a resilient data set (one that persists in memory and/or disk for the lifetime of the computation). The resident data set can be transformed using mapping (a term that comes from map/reduce but originates in functional programming language research). This approach is not to be confused with a related (but different) computational approach known as dataflow--a fine-grain parallel architecture that was the subject of much research in the 1980s (cite: Arvind and others), which focused on dataflow as a mechanism for triggering instructions. We also note that data flows are not to be confused with the compiler principle of data flow analysis, which is used to perform optimizations, including but not limited to strategies such as dead-code elimination, common subexpression elimination, and loop unrolling. 

%Also simply describe differences between implementation (e.g. lines of code).

%Out of core: Implicit in Spark

%NOTE: we need to clarify what we mean by \emph{dataflow.} Notably, it is a different from its meaning in \emph{compilers} and \emph{computer architecture}:
%\begin{itemize}
%\item
%  \href{https://en.wikipedia.org/wiki/Data-flow_analysis}{\emph{https://en.wikipedia.org/wiki/Data-flow\_analysis}}
%\item
%  https://en.wikipedia.org/wiki/Dataflow\_architecture
%\end{itemize}

%\paragraph{Project Resources}\label{project-resources}

%\textbf{Github:}
%\href{http://github.com/cchriste/dataflow}{\emph{http://github.com/cchriste/dataflow}}

%\textbf{Slack:}
%\href{https://dataflowanalysis.slack.com}{\emph{https://dataflowanalysis.slack.com}}

%\textbf{Google Docs:}
%\href{https://drive.google.com/folderview?id=0BxLkEMNd9q6FfmpRaFZXSGlPc0JsSDdVdndCUm83SzN6UnlLVEk5T3ZsZmJ0VEVGREtNTkE\&usp=sharing}{\emph{dataflow\_analysis}}

%\textbf{Dropbox:}
%\href{https://www.dropbox.com/sh/odsd9uxe1elbhbf/AAD8J1TGuFY1VHJl2oPdm5E0a?dl=0}{\emph{spark\_hpc}}




==> delete/narrative.tex <==
\section{About Apache Spark and Dataflows}
% TODO: We don't need to call this Narrative. Placeholder name.

Apache Spark is a general purpose cluster computing system similar to Hadoop. It provides a new data abstraction that facilitates fast sharing and history-based resilience, as well as an expanded set of data transformation and actions, in addition to traditional map-reduce. In addition, Spark provides a streaming processing abstraction as well as bindings to common processing languages such as GraphX, R, and MLlib.

Spark is \emph{lazy}, and this philosophy underlies much of its design. Computations will not be performed until their result is requested and data will not be consolidated or repartitioned unless explicitly requested.

\subsection{Submitting Spark Jobs on Cluster}
\label{running}

\subsubsection{Starting Spark in Cluster Mode on Cooley}

The following snippet shows how we start an ephemeral Spark cluster within our job submission script\footnote{Note that there are some minor differences from our actual version to improve formatting within the paper.}
\begin{lstlisting}[basicstyle=\ttfamily\small]
pushd $HOME/code/spark
cat $COBALT_NODEFILE > conf/slaves
cat $COBALT_NODEFILE >> $JOB_LOG
./sbin/start-all.sh
NODES=`wc -l conf/slaves | cut -d" " -f1`
popd

MASTER=`hostname`

ANL=cooley.pub.alcf.anl.gov
SPARK_STATUS_URL=http://$MASTER.$ANL:8000"
SPARK_MASTER_URI=spark://$MASTER:7077
SPARK_HOME=$HOME/code/spark
\end{lstlisting}

The job scheduler used on Cooley is Cobalt. When a Cobalt job script is submitted, it runs on the head node, after which services can be started on the head and other nodes in the allocation.

As shown above, a variable \texttt{\$COBALT\_NODEFILE} points to a file containing the hostnames that were allocated to the job. We use this list to populate \texttt{conf/slaves} in the Apache Spark configuration folder. Then we use the Apache Spark \texttt{start-all.sh} script to launch the Apache Spark master and worker daemons on the entire cluster.

Once Apache Spark is started in cluster mode, we now have the equivalent of a local cloud, albeit ephemeral, that we can use to run one or more Spark jobs. As shown above, variables are set so we can refer to the master URI. In the above, \texttt{\$MASTER} is the head node allocated by Cobalt. \texttt{spark://\$MASTER:7077} is what the Spark submit command (discussed next) will use to submit a Python or Java/Scala job for execution on the cluster. 

\subsubsection{Running a Spark Job on Cooley}

Once the Spark network is started, one or more actual Apache Spark jobs can be executed.

This excerpt shows how to run the Scala version of our benchmark on the ephemeral Apache Spark cluster we just created:

\begin{lstlisting}[basicstyle=\ttfamily\small]
BUILD=./target/scala-2.10
J=$BUILD/simplemap-spark-scala-assembly-1.0.jar
$SPARK_HOME/bin/spark-submit \
 --master $SPARK_MASTER_URI $J \
 --generate --blocks 128 --block_size 64 --nodes 1 \
 --nparts 1 --cores 12 \
 --json $JOB_JSON >> $JOB_LOG
\end{lstlisting}

We'll speak a bit to the parameters when discussing the performance study, but the most important thing, for now, is to observe that the variables set earlier are used to run the job in a relocatable way.

In the Scala version of our benchmark, a simple script is written to generate scripts to start Spark and run the benchmark-specific code for the parameter studies of interest. This allows for completely non-interactive execution of the benchmark study on Cooley, subject to available resources. Although this is mostly of interest to developers, we think this can be helpful to other researchers doing work with Spark in clustered environments, especially when they want to set up and tear down a Spark cluster for each job.

\subsubsection{Resilient Distributed Data}\label{resilient-distributed-data}

When a dataset is loaded by Spark, it becomes an immutable Resilient Distributed Data (RDD) collection. This abstraction allows the data to be treated as a whole when in fact it may
be partitioned across many nodes of a distributed system. Each partition also contains the history of transformations with which it was created,
called a \emph{lineage}, with which the partition can be recomputed if necessary, such as in the case of a node failure. This lineage is a more compact form of resiliency compared to data duplication as utilized by Hadoop.

An RDD is split into \emph{partitions} whose size is at minimum the size of a block on whatever storage device is being utilized (e.g. 32MB). Each partition is further divided into \emph{records}, typically a
single line for text processing, or an entire binary file for binary data. Binary data records can be explicitly specified. Large binary files will be broken down into multiple partitions only if these
partitions can themselves be divided into records.

Spark distributes the blocks/data among the workers, if it does at all. Apache Spark supports fault tolerance among the workers. For example, if a worker is lost, processing can continue. Although node failure rates are expected to be low in small-to-medium size clusters, larger clusters are more likely to see single node failures, thus making Apache Spark potentially compelling even in highly-reliable supercomputing clusters. As is well-known in the MPI community, attaining such functionality requires application-specific checkpointing and/or a fault-tolerant runtime, both of which incur significant overheads. With Apache Spark, the transparent support for fault tolerance allows the application code to be written without such overheads (at least in theory). While not the subject of this paper, we're intrigued by the potential to look at performance in future work, especially in the presence of one or two node failures.

\paragraph{Storage Levels}\label{storage-levels}

RDDs can be stored in memory, on disk, a combination of the two, or off heap (using Tachyon). MEMORY\_ONLY. In our experiments, we focus on RDDs that persist to RAM. We also have designed our experiments to consider out-of-core persistence strategies and spill rates (which we can simulate by multiplying the number of blocks, the number of partitions, or both).

Partitions that do not fit in memory will be recomputed from their history when they are needed. This recomputation is possible because RDDs are basically Scala immutable collections and are manipulated using map (to create a new RDD) and reduce (to gather results from nodes and apply a function between all pairs). 

In our benchmark, we are primarily considering mapping dataflow performance but also report initial results on reduce performance.

\paragraph{DISK\_ONLY}\label{diskux5fonly}

All partitions are stored on disk, just like Hadoop.

RDD partitions can be optionally replicated across up to two nodes. An RDD partition must be small enough to fit

\paragraph{Persistence}\label{persistence}

RDDs can be persisted in memory for fast access between successive
operations. This is particularly important for iterative algorithms that
reuse some intermediate result. An RDD will be persisted according to
its specified storage level. Caches are cleared according to a least
recently used policy, or manually using RDD.unpersist()

\paragraph{Input}\label{input}

In order to get binary data into spark, we use the binaryFiles or
binaryRecords SparkContext functions. Both will read a directory filled
with binary files. The first will create one record per file, while the
second will partition files into records of an explicitly stated number
of bytes. For example, the following line will create an RDD with
partitions containing records of size float{[}3{]}:

vecs = sc.binaryRecords(sys.argv{[}1{]}, 12)

The binary data is read into a string. If you want to use the data as a
numpy array, the numpy.fromstring function can be used:

arr= np.fromstring(vec, dtype=np.float32)

This function can be used by RDD.map in order to convert the string
records into numpy records:

data = vecs.map(parseVector)

\subsubsection{Streaming}\label{streaming-1}

How to run spark in streaming mode.

\subsubsection{Spark and Tachyon}\label{spark-and-tachyon}

How do they work together? Are the performance characteristics
different?

Is it the same as ceph on Magellan? (ask Dan Olsen about ceph)

\subsubsection{Pegasus}\label{pegasus}

todo

\subsubsection{MPI}\label{mpi}

todo: reference implementation

\subsection{System Architectures}
\label{system-architectures}

\subsubsection{Cooley}\label{cooley}

Cooley is a 225 Tflop cluster with 40TB memory, large shared disk (GPFS) + 355TB local scratch space per node.


\subsection{Sample Applications}\label{sample-applications}

\todo{I don't believe we are covering sample applications in this paper. All of that text can be found in the original google document, so I have removed it from this workshop paper..}



==> delete/performance.tex <==
\section{Performance}

We evaluate the potential of Spark in the analysis of large-scale scientific datasets. In this section we discuss performance results from the comparison of various Spark configurations with each other. For the purposes of comparison, we utilize a simple map example that transforms input data directly. We chose to concentrate on this example because it illustrates the most basic use of the map-reduce paradigm for data processing~\footnote{The Python version does map only, while the Scala version does map and reduce.}. The operations performed are simple calculations, very fast compared to the memory transfers involved in loading data.

\subsection{Infrastructure}

We utilize the Cooley visualization cluster at Argonne National Lab for our performance comparison. This system has 128 Infiniband-connected nodes, each with 12 Xeon cores, 384 MB system memory, and a 384 MB local SSD cache. 
\subsection{Spark}

Each node of Cooley is much more powerful and equipped with more memory than a typical cloud computing node and we leverage this in our tests, configuring the system to use 32 MB ram per spark process \todo{probably 32? is this a manual setting, I can't remember}. We scaled our testing from one to 16 nodes, utilizing from 12 to 192 cores, with one Spark process per core. Our Spark tests involve variation of block size, number of Spark processes, number of physical processor resources, and overall data size. We perform tests that load data from disk as well as generating data directly on the node.

\subsection{Python-based Experiments}

We first present the results of a set of strong and weak scaling experiments using a simple mapping application written in Python. While Python is not the native representation for Spark, the broad availability of analysis libraries makes it an appealing selection for scientific data processing. We later compare the results of our Python-based experiments with native Scala versions of the application. 

\textbf{Loading data from disk.} Our initial tests load data directly from shared storage using NFS-mounted directories on each node. The results of these tests for strong scaling can be seen in Figure~\ref{fig:strong-scaling-loaded}. The speedup as the number of nodes is increased is shown in Figure~\ref{fig:strong-scaling-speedup-loaded}. Note the maximum speedup reported is only 68.8\% efficient (11.98x) compared to the 16x resources provided. Both 64GB and 128GB data sizes exhibited the best scaling, while small data sizes (up to 8GB) were quickly overwhelmed by the overhead of distribution. Of the more massive data, the 2 TB case scaled at 60.3\% efficiency (9.64x), while data sizes between 256GB and 1024GB scaled slightly worse. \todo{in discussion we could speculate about this distribution, which is fascinating}

\begin{figure}[h]
\centering
\includegraphics[width=0.4\textwidth]{figures/strong_scaling_loaded}
\caption{Strong Scaling Loaded}
\label{fig:strong-scaling-loaded}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=0.4\textwidth]{figures/strong_scaling_speedup_loaded}
\caption{Strong Scaling Loaded}
\label{fig:strong-scaling-speedup-loaded}
\end{figure}

Our results for weak scaling of loaded data are shown in Figure~\ref{fig:weak-scaling-loaded}. The weak scaling tests using generated data show an obviously poor scaling when more nodes are added. Since the amount of computation is identical for each increment of nodes in this scenario, the time should remain about the same as the number of nodes is increased. Since larger jobs take more time, the implication is that loading the data itself does not scale well. 

\begin{figure}[h]
\centering
\includegraphics[width=0.4\textwidth]{figures/weak_scaling_loaded}
\caption{Weak Scaling Generated}
\label{fig:weak-scaling-loaded}
\end{figure}

\textbf{Generating data on node.} Since the weak scaling tests above indicated a diminished ability to scale as more data was loaded, we postulated that distributing the data among the nodes prior to beginning the job would likely result in better performance. Distributed file system such as HDFS or Tachyon\todo{introduce Tachyon and HDFS in background, cite appropriate work} provide exactly this sort of functionality, ideally enabling data to be loaded very near the computation. Although we performed preliminary tests using Tachyon, an in-memory distributed file system, we encountered some configuration issues and the results were not yet available at the time of this writing. Instead, we elected to generate data directly on the nodes. This generation simulates the use of an actual distributed file system and allows us to reason about the role of disk I/O in our previous experiments. 

The results of the tests for strong scaling using generated data can be seen in Figure~\ref{fig:strong-scaling-generated}. The speedup as the number of nodes is increased is shown in Figure~\ref{fig:strong-scaling-speedup-generated}. Note the maximum speedup reported in this new case is 93.6\% efficient (14.98x) of the 16x nodes used for the experiment. The 128GB data sizes once again exhibited the best scaling, while small data sizes were again less effective due to high system overhead compared to the amount of computation to be performed. The larger experiments up to 2 TB all scaled at least as well as the poorest of the group when data was being loaded, between 70\% and 80\% efficiency.

\begin{figure}[h]
\centering
\includegraphics[width=0.4\textwidth]{figures/strong_scaling_generated}
\caption{Caption Here}
\label{fig:strong-scaling-generated}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=0.4\textwidth]{figures/strong_scaling_speedup_generated}
\caption{Strong Scaling Speedup Generated}
\label{fig:strong-scaling-speedup-generated}
\end{figure}

Even more confirming of our suspicion that shared file resource contention is an issue for massive data processing using this system are the results of our weak scaling experiments using generated data, shown in Figure~\ref{fig:weak-scaling-generated}. This figure clearly illustrates almost perfect weak scaling as the number of nodes and amount of work are both linearly increased. This suggests the adoption of a distributed file system could be advantageous even for traditional MPI-based applications which read massive amounts of data. 

\begin{figure}[h]
\centering
\includegraphics[width=0.4\textwidth]{figures/weak_scaling_generated}
\caption{Weak Scaling Generated}
\label{fig:weak-scaling-generated}
\end{figure}

%cut: we have no data :) \subsection{Comparison with MPI \todo{cut?}}
 
%\todo{George, I don't think I ever got the MPI-based app working for an apples-to-apples comparison, and I don't see any data about it. Perhaps we should just make this paper about comparing spark, especially given the python vs scala angle. Otherwise, we (you) may have to scramble to get the mpi app working}

\todo{Cameron, I completely agree. We need to drop the MPI language, except to say that we considered the types of applications/flows that people do in MPI. This paper is only about Spark Python/Scala stuff, specifically benchmarking. Great!}

\subsection{Scala-based Experiments}

Figure~\ref{fig:mapshifttime} shows the results for map time. This is the time dedicated to creating the RDD and to persist it in memory (if available, of course).

Figure~\ref{fig:mapshifttime} shows the time to perform a global generate + shift on all of the vectors, using the cached RDD.

\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{figures/weak_scaling_scala}
% where an .eps filename suffix will be assumed under latex, 
% and a .pdf suffix will be assumed for pdflatex; or what has been declared
% via \DeclareGraphicsExtensions.
\caption{Generating synthetic data and applying a global operation, shift, to a large distributed array of vector data.}
\label{fig:mapshifttime}
\end{figure}

Figure~\ref{fig:avgtime} shows the time to perform a global average (reduce) on all of the vectors, using the cached RDD.

\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{figures/weak_scaling_scala_reduce}
% where an .eps filename suffix will be assumed under latex, 
% and a .pdf suffix will be assumed for pdflatex; or what has been declared
% via \DeclareGraphicsExtensions.
\caption{Performing a large reduce (global vector average) on a large, distributed array of vector data.}
\label{fig:avgtime}
\end{figure}


\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{figures/strong_scaling_scala}
\caption{Creating RDD of a large, distributed array of vector data and applying a shift mapping operation to the data}
\label{fig:scalastrong}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{figures/strong_scaling_scala_speedup}
\caption{Speedup when scaling: Creating RDD of a large, distributed array of vector data and applying a shift mapping operation to the data}
\label{fig:scalastrongspeedup}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{figures/strong_scaling_scala_reduce}
\caption{Performing a large reduce (global vector average) on a large, distributed array of vector data.}
\label{fig:scalareduce}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{figures/strong_scaling_scala_reduce_speedup}
\caption{Speedup when scaling: Performing a large reduce (global vector average) on a large, distributed array of vector data.}
\label{fig:scalareducespeedup}
\end{figure}





==> delete/references.tex <==
%
% The following two commands are all you need in the
% initial runs of your .tex file to
% produce the bibliography for the citations in your paper.
%\bibliographystyle{abbrv}
%\bibliography{sigproc}  % sigproc.bib is the name of the Bibliography in this case
% You must have a proper ".bib" file
%  and remember to run:
% latex bibtex latex latex
% to resolve all references
%
% ACM needs 'a single self-contained file'!
%
%APPENDICES are optional
%\balancecolumns
%of the document.
\subsection{References}



==> delete/relatedwork.tex <==
\section{Related Work}

\todo{Chiamov summary. Will likely have to shorten.}
There is growing interest in working with Apache Spark in traditional and high-performance clustering environments. This makes sense, considering that Apache Spark provides direct support for configuring a clustered mode. As well, there is also growing interest in understanding Apache Spark performance, especially when it comes to in and out of core execution.

Chaimov et al~\cite{Chaimov:2016:SSH:2907294.2907310} have done extensive work on porting Spark to large production HPC systems, specifically the Cray. Some key takeaways from their work include:

Similar to our work, they configure Spark to use local storage for the shuffle stage, which improves scalability in their problem to 10,000 cores. Our micro-benchmark can be used in such an environment, but our testbed limits us in this study to 126 * 12 cores.

Similar to our work, they also evaluated a configuration with storage attached closer to compute nodes for I/O acceleration. Our paper is mostly focused on large, generated data sets, but we have also evaluated I/O from the shared disk and experienced similar results.

The authors uncovered several scaling issues on HPC systems, which would likely be worse on lower-performing clusters. Fixing the YARN resource manager and improving the block management in the shuffle block manager will benefit performance. Our experiments have mostly been confined to being careful with persistence schemes, especially with how data are serialized (especially on the Java side, where you want to avoid serializing complex object hierarchies).

Slightly different focus than our paper but addresses lower-level aspects that could radically boost performance. We're interested in what we can do with the out-of-box Spark experience and limiting tuning to the configuration file itself (e.g. using scratch storage allows us to get fast disks as done in this paper).

\todo{Matrix factorization at scale. This is a good paper with a bit different focus but certainly one that helps to establish interest in what we're doing.}

Gittens et al~\cite{DBLP:journals/corr/GittensDRRGKLMC16} have done a recent study comparing MPI/C++ and Apache Spark Versions. 

In this work, the authors developed three different parallel versions of matrix factorizations and apply them to TB (terabyte) size data sets--on the same scale as our experiments.

Their testbed is the Cray XC40 with up to 1600 nodes. We're currently limited to 128 in our testbed (the only computer where we can run full Java stack code). 

Their findings confirm a performance gap between MPI/C++ and Apache Spark, which is expected.  The performance gaps are attributable to task-related overheads. In addition, serialization can play a major role, even when data are persisted to RAM. Our study is a bit more focused on strong/weak scaling in the presence of these overheads.

One thing not discussed in this paper is developer productivity, in particular the development effort to create the MPI version vs. the Apache Spark version. We have found that the development time for both our Python and Scala versions of the benchmark to be short, amounting to a few lines of code for each phase of the computation. We also did not find any information about strong vs. weak scaling results in the paper, which is more focused on understanding the low-level issues (task execution timeline) and performance overheads within a computation.

In any event, this paper gives us encouragement that large-scale data processing can work at scale. On our cluster of fat compute nodes, strong and weak scaling results are encouraging.


==> delete/summary.tex <==
\section{Summary}



==> old-benchmark-text.tex <==
\section{Benchmarking}

\todo{It will benefit us to describe our benchmark comprehensively in a single (sub-)section rather than have pieces of its description in many places. There is a now a reference to this section in the Intro when the benchmark we created is introduced.}

\todo{GKT: I completely agree with this comment. It is part of the plan. We will then be able to simplify the presentation of the overall results as well. In fact, that will be necessary. Thanks for thse great comments, Cameron!}

%% We'll move things around later
%\input{benchmarks.tex}

%%% PERFORMANCE %%%%
\section{Performance}

We evaluate the potential of Spark in the analysis of large-scale scientific datasets. In this section we discuss performance results from the comparison of various Spark configurations with each other. For the purposes of comparison, we utilize a simple map example that transforms input data directly. We chose to concentrate on this example because it illustrates the most basic use of the map-reduce paradigm for data processing~\footnote{The Python version does map only, while the Scala version does map and reduce.}. The operations performed are simple calculations, very fast compared to the memory transfers involved in loading data.

\subsection{Infrastructure}

We utilize the Cooley visualization cluster at Argonne National Lab for our performance comparison. This system has 128 Infiniband-connected nodes, each with 12 Xeon cores, 384 MB system memory, and a 384 MB local SSD cache. 
\subsection{Spark}

Each node of Cooley is much more powerful and equipped with more memory than a typical cloud computing node and we leverage this in our tests, configuring the system to use 32 GB RAM per spark process. We scaled our testing from one to 16 nodes, utilizing from 12 to 192 cores, with one Spark process per core. Our Spark tests involve variation of block size, number of Spark processes, number of physical processor resources, and overall data size. We perform tests that load data from disk as well as generating data directly on the node.

\subsection{Python-based Experiments}

We first present the results of a set of strong and weak scaling experiments using a simple mapping application written in Python. While Python is not the native representation for Spark, the broad availability of analysis libraries makes it an appealing selection for scientific data processing. We later compare the results of our Python-based experiments with native Scala versions of the application. 

\textbf{Loading data from disk.} Our initial tests load data directly from shared storage using NFS-mounted directories on each node. The results of these tests for strong scaling can be seen in Figure~\ref{fig:strong-scaling-loaded}. The speedup as the number of nodes is increased is shown in Figure~\ref{fig:strong-scaling-speedup-loaded}. Note the maximum speedup reported is only 68.8\% efficient (11.98x) compared to the 16x resources provided. Both 64GB and 128GB data sizes exhibited the best scaling, while small data sizes (up to 8GB) were quickly overwhelmed by the overhead of distribution. Of the more massive data, the 2 TB case scaled at 60.3\% efficiency (9.64x), while data sizes between 256GB and 1024GB scaled slightly worse.

\begin{figure}[h]
\centering
\includegraphics[width=0.4\textwidth]{figures/strong_scaling_loaded}
\caption{Strong Scaling Loaded}
\label{fig:strong-scaling-loaded}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=0.4\textwidth]{figures/strong_scaling_speedup_loaded}
\caption{Strong Scaling Loaded}
\label{fig:strong-scaling-speedup-loaded}
\end{figure}

Our results for weak scaling of loaded data are shown in Figure~\ref{fig:weak-scaling-loaded}. The weak scaling tests using generated data show an obviously poor scaling when more nodes are added. Since the amount of computation is identical for each increment of nodes in this scenario, the time should remain about the same as the number of nodes is increased. Since larger jobs take more time, the implication is that loading the data itself does not scale well. 

\begin{figure}[h]
\centering
\includegraphics[width=0.4\textwidth]{figures/weak_scaling_loaded}
\caption{Weak Scaling Generated}
\label{fig:weak-scaling-loaded}
\end{figure}

\textbf{Generating data on node.} Since the weak scaling tests above indicated a diminished ability to scale as more data was loaded, we postulated that distributing the data among the nodes prior to beginning the job would likely result in better performance. Distributed file system such as HDFS~\cite[hdfs] or Tachyon~\cite{tachyon} provide exactly this sort of functionality, ideally enabling data to be loaded very near the computation. Although we performed preliminary tests using Tachyon, an in-memory distributed file system, we encountered some configuration issues and the results were not yet available at the time of this writing. Instead, we elected to generate data directly on the nodes. This generation simulates the use of an actual distributed file system and allows us to reason about the role of disk I/O in our previous experiments. 

The results of the tests for strong scaling using generated data can be seen in Figure~\ref{fig:strong-scaling-generated}. The speedup as the number of nodes is increased is shown in Figure~\ref{fig:strong-scaling-speedup-generated}. Note the maximum speedup reported in this new case is 93.6\% efficient (14.98x) of the 16x nodes used for the experiment. The 128GB data sizes once again exhibited the best scaling, while small data sizes were again less effective due to high system overhead compared to the amount of computation to be performed. The larger experiments up to 2 TB all scaled at least as well as the poorest of the group when data was being loaded, between 70\% and 80\% efficiency.

\begin{figure}[h]
\centering
\includegraphics[width=0.4\textwidth]{figures/strong_scaling_generated}
\caption{Caption Here}
\label{fig:strong-scaling-generated}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=0.4\textwidth]{figures/strong_scaling_speedup_generated}
\caption{Strong Scaling Speedup Generated}
\label{fig:strong-scaling-speedup-generated}
\end{figure}

Even more confirming of our suspicion that shared file resource contention is an issue for massive data processing using this system are the results of our weak scaling experiments using generated data, shown in Figure~\ref{fig:weak-scaling-generated}. This figure clearly illustrates almost perfect weak scaling as the number of nodes and amount of work are both linearly increased. This suggests the adoption of a distributed file system could be advantageous even for traditional MPI-based applications which read massive amounts of data. 

\begin{figure}[h]
\centering
\includegraphics[width=0.4\textwidth]{figures/weak_scaling_generated}
\caption{Weak Scaling Generated}
\label{fig:weak-scaling-generated}
\end{figure}

\subsection{Scala-based Experiments}

In addition to Python, we also conducted experiments by porting our Python benchmark to Scala using the best available libraries that support numerical methods. We started with the Breeze~\cite{BreezeScala}, which is a core library used in the ScalaNLP (Scala Natural Language Processing) framework. (It is also a core library used in Apache Spark itself.)

\textbf{Comparing to Python version} The Scala benchmark supports all of the core features of the Python benchmark, including our ability to explore disk-based performance. Based on our initial results with Apache Spark and the shared GPFS filesystem, we decided to focus our energy on understanding how well Scala does compared to Python for distributed generated data sets. We also took advantage of the initial conclusion that 64MB block sizes are also a \emph{sweet spot} of sorts when it comes to understanding strong and weak scaling performance.

\textbf{Changes to Spark configuration for Java} Because our code is 100\% Java (Scala being a JVM language), we had to make a few changes in order to test Scala performance. Whereas the Python version can more or less rely upon Apache Spark's default configuration, we needed to configure the driver and executor (Spark's terms for what runs on the master and worker nodes) to use most of the available memory on the nodes. Because our workers need the most memory, we set this to 320GB.~\footnote{It should have been set higher as our performance charts clearly show. If our paper is accepted, we'll re-run these experiments.}  To be clear, Scala and Java require the use of JVM-managed memory, whereas the Python version actually uses unmanaged memory outside of the JVM running Spark itself.

\textbf{Other subtle differences} There are other subtle differences to how we developed the Scala version, this being owed to the developer (Thiruvathukal) wanting to get a more granular idea of how lazy evaluation plays a role, since this is a prevalent feature when working with Scala. 

The Scala version computes the times separately for the distributed data creation/generation, the mapped computation, and the reduced computation. At each of the first two stages, we also force a cache on the result to ensure that it is fully computed. Otherwise, it is not a fair comparison to what is happening in the Python version. 


\textbf{Other Java/Scala nuisances}
One issue that continues to plague Java (and Scala) is the 32-bit restriction on array sizes. This only affects our benchmark when we try to run with extremely large data sizes. At the same time, we don't want to write different code for when there are 32-bit and 64-bit indices required.

For the purpose of benchmarking, we need to wrap the dense vector representation of our benchmark data using an ordinary Scala (outer) array. This has the end result of putting the Scala code at a theoretical disadvantage, but our initial charts show that the Scala version does have better overall execution times, owing to the \emph{compiled} nature of Java code in general. In addition, the Breeze library we are using actually has support for native code, similar to NumPy in Python. So it is clear that the performance should be on par (not worse) at a minimum, given that native code is used when we need to perform operations on array structures.

\textbf{Initial Scala Results}

The results for strong scaling are shown in figure \ref{fig:scalastrong}. The speedup as the number of nodes is increased is shown in \ref{fig:scalastrongspeedup}. Contrasted with the Python version, we are experiencing some issues at the 64 GiB and 128 GiB sizes. In looking at our performance logs, we notice that we are experiencing a higher rate of data spilling when working with larger arrays, which speaks to a need to up the JVM memory in our executors. Nevertheless, we're encouraged by Scala's performance. Note that our time scale tops out at 4000 seconds for Scala and Breeze but is close to 10000 for Python and NumPy. We attribute these differences, however, not to the innate performance of each library itself but the overheads also associated with Apache Spark firing up Python for RDD processing. Clearly, further study is required.

Figure \ref{fig:mapshifttime} shows the results of our weak scaling experiments. Similar to the Python version, as the number of nodes and amount of work are linearly increased, we see similar (promising) results. Execution time at the high end (128 GiB) is generally better than the Python version.

We stress that these results are initial, and it is likely that the Java version is experiencing issues that require more study in future work. Our logs reveal data spilling happening, which is probably not occurring at all in the Python version, and there are likely more interactions with the garbage collector in Java. Nevertheless, we are encouraged by what is possible without doing too much tweaking. The initial results for Python and Scala versions of our benchmark clearly illustrate that promising scaling is possible.~\footnote{And we expect that we would have even better results for Scala by the time we present our paper at the workshop.}


\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{figures/weak_scaling_scala}
% where an .eps filename suffix will be assumed under latex, 
% and a .pdf suffix will be assumed for pdflatex; or what has been declared
% via \DeclareGraphicsExtensions.
\caption{Generating synthetic data and applying a global operation, shift, to a large distributed array of vector data.}
\label{fig:mapshifttime}
\end{figure}

Figure~\ref{fig:avgtime} shows the time to perform a global average (reduce) on all of the vectors, using the cached RDD.

\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{figures/weak_scaling_scala_reduce}
% where an .eps filename suffix will be assumed under latex, 
% and a .pdf suffix will be assumed for pdflatex; or what has been declared
% via \DeclareGraphicsExtensions.
\caption{Performing a large reduce (global vector average) on a large, distributed array of vector data.}
\label{fig:avgtime}
\end{figure}


\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{figures/strong_scaling_scala}
\caption{Creating RDD of a large, distributed array of vector data and applying a shift mapping operation to the data}
\label{fig:scalastrong}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{figures/strong_scaling_scala_speedup}
\caption{Speedup when scaling: Creating RDD of a large, distributed array of vector data and applying a shift mapping operation to the data}
\label{fig:scalastrongspeedup}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{figures/strong_scaling_scala_reduce}
\caption{Performing a large reduce (global vector average) on a large, distributed array of vector data.}
\label{fig:scalareduce}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{figures/strong_scaling_scala_reduce_speedup}
\caption{Speedup when scaling: Performing a large reduce (global vector average) on a large, distributed array of vector data.}
\label{fig:scalareducespeedup}
\end{figure}

